Position Prediction as an Effective Pretraining Strategy

Transformers have gained increasing popularity in a wide range of applications, including Natural Language Processing (NLP), Computer Vision and Speech Recognition, because of their powerful representational capacity. However, harnessing this representational capacity effectively requires a large amount of data, strong regularization, or both, to mitigate overfitting. Recently, the power of the Transformer has been unlocked by self-supervised pretraining strategies based on masked autoencoders which rely on reconstructing masked inputs, directly, or contrastively from unmasked content. This pretraining strategy which has been used in BERT models in NLP, Wav2Vec models in Speech and, recently, in MAE models in Vision, forces the model to learn about relationships between the content in different parts of the input using autoencoding related objectives. In this paper, we propose a novel, but surprisingly simple alternative to content reconstruction~-- that of predicting locations from content, without providing positional information for it. Doing so requires the Transformer to understand the positional relationships between different parts of the input, from their content alone. This amounts to an efficient implementation where the pretext task is a classification problem among all possible positions for each input token. We experiment on both Vision and Speech benchmarks, where our approach brings improvements over strong supervised training baselines and is comparable to modern unsupervised/self-supervised pretraining methods. Our method also enables Transformers trained without position embeddings to outperform ones trained with full position information.

==> speech_table_librispeech.tex <==
\begin{table*}[t!]
\caption{
Comparison with other sup, semi- and unsupervised methods on Librispeech (100h sup, the rest unsup).
\label{tab:speech_resuts}}
% \begin{scriptsize}
\begin{center}
\setlength\tabcolsep{5pt} 
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}cccccccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Stride} & \multirow{2}{*}{Tokens} & \multirow{2}{*}{Criterion} & \multirow{2}{*}{LM} & \multicolumn{2}{c}{Dev WER} & \multicolumn{2}{c}{Test WER} & \multicolumn{3}{c}{Compute Resources} \\
% Training Time & \multirow{2}{*}{Resources} \\
\cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-12}
 &  & & & & clean        & other        & clean    & other  & Train Time (Days) & \# G/TPUs & G/TPU-days \\
\midrule
\multirow{3}{*}{Sup. baseline} & \multirow{3}{*}{30ms} & \multirow{3}{*}{letters} & \multirow{3}{*}{CTC} & - & 6.2 & 16.8 & 6.2 & 16.8 \\
 & & & & word 4-gram & 4.1 & 12.4 & 4.5 & 12.7 \\
 & & & & \, \, + rescoring & 3.3 & 10.9 & 3.7 & 11.4  \\
 \midrule
  \multirow{2}{*}{IPL~\cite{xu2020iterative}} &  \multirow{2}{*}{80ms} & \multirow{2}{*}{5k wp} & \multirow{2}{*}{CTC} & - & 5.5 & 9.3 & 6.0 & 10.3 & \multirow{2}{*}{3} & \multirow{2}{*}{64~GPUs} & \multirow{2}{*}{192} \\
 & & & & \, \, + rescoring & 5.0 & 8.0 & 5.6 & 9.0 \\
\midrule
 \multirow{2}{*}{Improved T/S~\cite{park2020improved}} &  \multirow{2}{*}{-} & \multirow{2}{*}{16k wp} & \multirow{2}{*}{S2S} & - & 4.3 & 9.7 & 4.5 & 9.5 & \multirow{2}{*}{10 $\times$ 5} & \multirow{2}{*}{32~TPUs} & \multirow{2}{*}{1600} \\
  & & & & LSTM & 3.9 & 8.8 & 4.2 & 8.6 \\
\midrule
 \multirow{3}{*}{wav2vec~2.0~\cite{baevski2020wav2vec}} &  \multirow{3}{*}{20ms} & \multirow{3}{*}{letters} & \multirow{3}{*}{CTC} & - & 4.6 & 9.3 & 4.7 & 9.0  & \multirow{3}{*}{2.3} & \multirow{3}{*}{128~GPUs} & \multirow{3}{*}{294.4} \\
 & & & & word 4-gram & 2.3 & 5.7 & 2.8 & 6.0  \\
 & & & & word Transf. & 2.1 & 4.8 & 2.3 & 5.0 \\
\midrule
 \multirow{3}{*}{slimIPL~\cite{likhomanenko2021slimipl}} & \multirow{3}{*}{30ms} & \multirow{3}{*}{letters} & \multirow{3}{*}{CTC} & - & 3.7 & 7.3 & 3.8 & 7.5  & \multirow{3}{*}{5.2} & \multirow{3}{*}{16~GPUs} & \multirow{3}{*}{83.2} \\
 & & & & word 4-gram & 2.8 & 5.6 & 3.1 & 6.1 \\
 & & & & \, \, + rescoring & 2.2 & 4.6 & 2.7 & 5.2  \\
 \midrule
 \multirow{2}{*}{Our sup. baseline} & \multirow{2}{*}{30ms} & \multirow{2}{*}{letters} & \multirow{2}{*}{CTC} & - & 6.6 & 18.4 & TBD & TBD  & \multirow{2}{*}{TBD} & \multirow{2}{*}{8~GPUs} & \multirow{2}{*}{TBD} \\
 & & & & word 4-gram & TBD & TBD & TBD & TBD \\
 \midrule
 \multirow{2}{*}{MP3} & \multirow{2}{*}{30ms} & \multirow{2}{*}{letters} & \multirow{2}{*}{CTC} & - & TBD & TBD & TBD & TBD  & \multirow{2}{*}{TBD} & \multirow{2}{*}{8~GPUs} & \multirow{2}{*}{TBD} \\
 & & & & word 4-gram & TBD & TBD & TBD & TBD \\
 \bottomrule
\end{tabular}
}
\end{center}
% \end{scriptsize}
\end{table*}
